Self-Contradictory Reasoning Evaluation and Detection

In a plethora of recent work, large language models (LLMs) demonstrated impressive reasoning ability, but many proposed downstream reasoning tasks only focus on final answers. Two fundamental questions persist: 1) how consistent is the reasoning, and 2) can models detect unreliable reasoning? In this paper, we investigate self-contradictory (Self-Contra) reasoning, where the model reasoning does not support its answers. To answer 1), we define and assess the Self-Contra rate across three datasets and delve into finer-grained categories of Self-Contra reasoning. We find that LLMs often contradict themselves in reasoning tasks involving contextual information understanding or commonsense. The model may generate correct answers by taking shortcuts in reasoning or overlooking contextual evidence, leading to compromised reasoning. For 2), we task the state-of-the-art model GPT-4 with identifying Self-Contra reasoning and finer-grained fallacies. We find that finer-grained categories enhanced detection can improve GPT-4's ability to detect Self-Contra. However, it is only able to detect Self-Contra with a 52.2% F1 score, much lower compared to 66.7% for humans. Our results indicate that current LLMs lack the robustness necessary for reliable reasoning and we emphasize the urgent need for establishing best practices in comprehensive reasoning evaluations beyond pure performance-based metrics.

==> sections/6.1_pov-method.tex <==

\sca rate quantifies the inconsistency in LLM reasoning, and further reveals finer-grained categories of \sca reasoning. On the other hand, the categories of failures are not connected to model robustness or possible causes. 
%\Ziyi{should we put the confidence thing in the automatic evaluation?}  \jz{why is this related to "confidence"? Are you saying "reliabity" or "robustness of LLM reasoning"?} 
We investigate \sca behavior with multi-turn interactions to gain better insight. Since humans can detect errors in natural language reasoning when they consider answers from multiple perspectives, we similarly probe model reasoning by asking LLMs to reason from multiple perspectives.
%\jz{Can we add back the wording of humans might detect the errors in their answers with multiple perspectives and inspired by this, we do the same setting on LLMs? Otherwise I feel introducing of this POV of "model utilizes a given context" is still a little bit weak. } 
For this, we experiment with WinoBias anti-set. As illustrated in Table \ref{tab:pov_prompt}, we ask GPT-3.5\footnote{We made 600 calls for experiments with temperature 0.}to consider the prompt with the pronoun from one perspective, or ``point of view'' and to reason through it. Then, we ask the model to consider the prompt from the other perspective. Finally, we ask the model to choose a more likely perspective and provide reasoning. Since LLMs are sensitive to context, we also switch the order of perspectives. Some illustrative examples are shown in Appendix \ref{sec:pov_examples}, Table \ref{tab:pov_examples} as well as overview of results are summarized in Table \ref{tab:pov-results}. 
POV experiments accuracies were similar for both good and bad reasoning. Further analysis of POV results possibly suggest that the model reasoning may not remain self-consistent beyond one-turn. %\jz{should move these results (starting from Table 16.. to Sec. 5.2}


%\jz{what message can we get from those tables?}
%\Ziyi{better to cite this jung2022maieutic, people might ask}

==> sections/6.2_pov_results.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/cm.png}
    \caption{Confusion Matrix of POV Predictions: \textbf{RR} indicates \textbf{R}ight reasoning \textbf{R}ight prediction, \textbf{WW} indicates \textbf{W}rong reasoning \textbf{W}rong prediction, and \textbf{SC} indicates self-contradictory labels such as \textbf{R}ight reasoning \textbf{W}rong prediction and visa versa.} 
    % \jz{can you make the x-axis on the top of the figure?} \igl{i'm trying to rotate it, but struggling ;;}
    \label{fig:pov-cm}
\end{figure}


We first draw comparisons between POV predictions and human judgements. We computed the confusion matrix for POV results and prediction categories, as shown in Figure \ref{fig:pov-cm}. 
In this setting, we count the reasoning as correct only if the model gives correct answers for both turns. \sca is defined as either correct reasoning leading to wrong prediction (Type 1) or wrong reasoning leading to correct prediction (Type 2). %\jz{how do you define SC in POV?} 
We see that the POV reasoning is able to identify RR reasonably well, but there's significant disconnect between human judgements and model reasoning in other categories. The model is unable to identify \sca categories annotated by humans, and moreover, the model seems to be overly reliant on the correctness of prediction rather than reasoning.

\begin{table}[h!]
\centering
\scalebox{0.68}{
\begin{tabular}{lrr}
\toprule
\textbf{\makecell[l]{Annotated\\ labels}}&\textbf{\makecell[r]{POV Reasoning\\Correctness}}&\textbf{\makecell[r]{POV Prediction\\Correctness}}\\
\toprule
\textbf{RR} &0.23& 0.17\\
\textbf{Type 1 (RW)} & -0.19& -0.12\\
\textbf{Type 2 (WR)} & 0.25&0.18\\
\textbf{WW} & -0.35&-0.25\\
\bottomrule
\end{tabular}}
\caption{Spearman Correlation between POV reasoning and human annotations.}
\label{tab:corr-pov}
\end{table}

To parse this further, we calculate the Spearman correlation between POV reasoning and predictions vs. one-hot encoded human annotated labels as shown in Table \ref{tab:corr-pov}. 
We see that the POV predictions are correlated with human labels, whereas the POV reasoning correctness is inversely correlated with human reasoning predictions in \sca categories. For instance, the annotated \sca Type 1 category (Right Reasoning, Wrong Prediction) is expectantly negatively correlated with POV predicted correctness, but falsely, negatively correlated with with POV reasoning correctness despite having right reasoning.
%\Ziyi{bit hard to follow} 
This may indicate that the model is overly reliant on the correctness of the prediction, and the model sometimes misleadingly assumes how correct its own reasoning is to follow its prediction.
%\jz{after reading this section, I don't know I can connect it well with previous sections.}

==> tables/sec2_result_all.tex <==
\begin{table*}[h!]
\centering
\scalebox{0.75}{
\begin{tabular}{lllrrrr}
\toprule
\textbf{Models}&\textbf{Dataset}&\textbf{Metrics}&\textbf{Zero-shot(R)}&\textbf{Zero-shot(A)}&\textbf{Few-shot(R)}&\textbf{Few-shot(A)}\\
\midrule
\multirow{6}{*}{\textbf{GPT3.5}}&\multirow{2}{*}{\textbf{WinoBias}}&
\textsc{Acc}&0.56&0.56&0.72&0.72\\
& &\textsc{Self-Contra Rate}&0.34&0.28&0.38&0.32\\
% \midrule
% \multirow{2}{*}{\textbf{WinoGender}}&
% \textsc{Acc}&x.xx&x.xx&x.xx&x.xx&x.xx\\
% &\textsc{Self-Contra Rate}&x.xx&x.xx&x.xx&x.xx&x.xx\\
\cmidrule{2-7}
& \multirow{2}{*}{\textbf{WinoGender}}&
\textsc{Acc}&0.80&0.86&0.90&0.96\\
& &\textsc{Self-Contra Rate}&0.40&0.60&0.22&0.26\\
\cmidrule{2-7}
&\multirow{2}{*}{\textbf{WinoGrande}}&
\textsc{Acc}&0.64&0.74&0.80&0.78\\
& &\textsc{Self-Contra Rate}&0.16&0.30&0.20&0.18\\


\midrule
\multirow{6}{*}{\textbf{Claude3}}&\multirow{2}{*}{\textbf{WinoBias}}&
\textsc{Acc}&0.90&0.78&0.86&0.86\\
& &\textsc{Self-Contra Rate}&0.64&0.10&0.08&0.10\\
% \midrule
% \multirow{2}{*}{\textbf{WinoGender}}&
% \textsc{Acc}&x.xx&x.xx&x.xx&x.xx&x.xx\\
% &\textsc{Self-Contra Rate}&x.xx&x.xx&x.xx&x.xx&x.xx\\
\cmidrule{2-7}
& \multirow{2}{*}{\textbf{WinoGender}}&
\textsc{Acc}&0.96&0.86&0.98&1.00\\
& &\textsc{Self-Contra Rate}&0.20&0.12&0.06&0.02\\
\cmidrule{2-7}
&\multirow{2}{*}{\textbf{WinoGrande}}&
\textsc{Acc}&0.92&0.94&0.98&1.00\\
& &\textsc{Self-Contra Rate}&0.06&0.06&0.04&0.04\\



\midrule
\multirow{6}{*}{\textbf{Mistral 7B}}&\multirow{2}{*}{\textbf{WinoBias}}&
\textsc{Acc}&0.74&0.44&0.46&0.36\\
& &\textsc{Self-Contra Rate}&0.46&0.48&0.44&0.50\\
% \midrule
% \multirow{2}{*}{\textbf{WinoGender}}&
% \textsc{Acc}&x.xx&x.xx&x.xx&x.xx&x.xx\\
% &\textsc{Self-Contra Rate}&x.xx&x.xx&x.xx&x.xx&x.xx\\
\cmidrule{2-7}
& \multirow{2}{*}{\textbf{WinoGender}}&
\textsc{Acc}&0.78&0.82&0.94&0.84\\
& &\textsc{Self-Contra Rate}&0.26&0.42&0.32&0.26\\
\cmidrule{2-7}
&\multirow{2}{*}{\textbf{WinoGrande}}&
\textsc{Acc}&0.68&0.72&0.66&0.74\\
& &\textsc{Self-Contra Rate}&0.30&0.24&0.30&0.26\\
% \midrule
% \multirow{2}*{\textbf{Overall}}&
% &\textsc{Acc}&0.78 &0.74 &0.81 &0.81 \\
% & &\textsc{Self-Contra}&0.31 & 0.29& 0.22& 0.22\\

\bottomrule
\end{tabular}}
\caption{Accuracy and \sca rate results. The evaluation is done by humans. (R) means reasoning first and (A) means answer first. The overall \sca rate and accuracy for zero-shot prompting are 0.30 and 0.76, while for few-shot prompting, they are 0.22 and 0.81. }
\label{tab:results}

\end{table*}
